Redefining non-IID Data in Federated Learning for Computer Vision Tasks: Migrating from Labels to Embeddings for Task-Specific Data Distributions

Federated Learning (FL) has emerged as one of the prominent paradigms for distributed machine learning (ML). However, it is well-established that its performance can degrade significantly under non-IID (non-independent and identically distributed) data distributions across clients. To study this effect, the existing works predominantly emulate data heterogeneity by imposing label distribution skew across clients. In this paper, we show that label distribution skew fails to fully capture the data heterogeneity in computer vision tasks beyond classification, exposing an overlooked gap in the literature. Motivated by this, by utilizing pre-trained deep neural networks to extract task-specific data embeddings, we define task-specific data heterogeneity through the lens of each vision task and introduce a new level of data heterogeneity called embedding-based data heterogeneity. Our methodology involves clustering data points based on embeddings and distributing them among clients using the Dirichlet distribution. Through extensive experiments, we evaluate the performance of different FL methods under our revamped notion of data heterogeneity, introducing new benchmark performance measures to the literature. For instance, across seven representative computer vision tasks, our embedding-based heterogeneity formulation leads to up to around 60% increase in the observed loss under FedAvg, indicating that it more accurately exposes the performance degradation caused by data heterogeneity. We further unveil a series of open research directions that can be pursued. (Code: https://github.com/KasraBorazjani/task-perspective-het.git)

==> Backup/intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/0_abstract.tex <==
\begin{abstract}
Federated Learning (FL) enables collaborative model training across decentralized clients without sharing raw data, thereby preserving privacy. While FL has traditionally focused on classification tasks using Dirichlet distributions to simulate data heterogeneity, this label-based heterogeneity approach may not effectively capture the challenges in vision tasks like surface normal or depth estimation. These tasks demand nuanced data representations, as they often interpret the same dataset differently depending on task-specific requirements. For instance, images of indoor scenes may exhibit heterogeneity in surface orientation but remain spatially consistent across different clients, which affects FL performance differently depending on the task. To address this, we propose a task-specific framework for introducing data heterogeneity in FL for non-classification vision tasks. Our approach utilizes pretrained task-specific deep neural networks (DNNs) to generate embeddings from low- and high-level features of the data. This representation undergoes clustering, and a Dirichlet distribution then allocates data to clients based on cluster assignments, ensuring a heterogeneity measure that aligns with each task’s unique perspective. This framework promotes a more accurate analysis of FL’s efficacy in vision tasks, enhancing FL model robustness under varying levels of task-specific heterogeneity.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Federated Learning (FL) has emerged as a promising paradigm for distributed machine learning (ML), enabling clients to collaboratively train models without sharing raw data, thus preserving user privacy. This approach offers an alternative to traditional centralized ML techniques, where data must be transferred to a central server, often resulting in significant communication overhead and privacy concerns. In FL, model training is conducted over multiple global rounds, with each round consisting of two main steps: (i) clients perform local model training on their local dataset, typically using several iterations of stochastic gradient descent (SGD), and then send their updated models to a central server, and (ii) the server aggregates the local models (e.g., through averaging) into a global model and broadcasts it back to clients to initiate the next round of local training. 

Implementing FL in practice faces unique challenges, largely due to the \textit{inherent non-i.i.d. (non-independent and identically distributed) nature of data across clients}. This 
data heterogeneity has a significant impact on FL performance. Specifically, as non-i.i.d.-ness (or data heterogeneity) increases, local models of clients become biased toward their local datasets, negatively affecting the overall convergence and accuracy of the global model. 
% Thus, proposing robust FL to data heterogeneity is a major research area [CITE]. 
Effectively evaluating the robustness of FL algorithms necessitate examining how data heterogeneity influences FL performance. Nevertheless, real-world FL deployment is often impractical due to high costs, restricted network access, limited client availability, and privacy concerns. Simulation techniques, therefore, have become a key approach for replicating real-world data heterogeneity, as they provide a controlled environment for experimentation, enabling systematic analysis of how varying heterogeneity levels influence FL model performance.


% This data heterogeneity arises from different local contexts, user behaviors, and device environments, making it difficult to achieve robust, generalizable model performance. Addressing data heterogeneity is therefore crucial for the effectiveness and convergence of FL models.
% Motivation for simulating data heterogeneity. In real world this heterogeneity exist, but in simulation it is a major task that can affect the efficiency of algorithms,,

When FL first emerged as a decentralized ML paradigm, researchers initially distributed data points based on their labels across different clients as a way to represent the non-i.i.d nature of data in FL and became widely used method to simulate data heterogeneity in early FL research. For example, in the MNIST dataset, rather than giving each client a fully representative dataset of the global dataset, clients would receive only a subset of the available labels. As the number of labels per clients decreases, each client's dataset become less representative to the global dataset. This increases the divergence between local and global data distributions, leading to local model bias. This is mainly because local models become biased to the limited label available locally at each clients and converge towards solution that are optimal only for their specific data distribution. As a result, aggregation of these biased local models hampers the global model accuracy, robustness, and convergence rate.

% While the above approach introduces some degree of variation, it does not capture the full complexity of heterogeneity observed in real applications. To achieve finer control over data heterogeneity, recent research have introduced the use of Dirichlet distribution to disperse data points among clients, which enables a more gradual heterogeneity in label distribution across clients by fine-tuning the concentration parameters. Nevertheless, current Dirichlet-based approaches are limited to label-based heterogeneity, which restricts their applicability in more complex FL scenarios, such as vision tasks.



While the above approaches introduce some degree of data heterogeneity, there was a pressing need for mathematical and unified approaches to introduce and measure the level of heterogeneity. A major step in this direction was taken by introducing Dirichlet distributions for dispersing data points among clients in FL, enabling gradual heterogeneity in label distributions by fine-tuning Dirichlet concentration parameters. This methodology inherently induces label-based heterogeneity which makes it naturally a good fit for classification task. However, this label-based data heterogeneity may not be a prefect match for other vision tasks, such as surface normal estimation, depth estimation, and object detection, which are not necessarily sensitive to the labels of data points. Building on this intuition, in this paper, we propose the following fundamental claim (demonstrated in Fig.~\ref{}):

\begin{quote}
    Most existing studies on FL simulate data heterogeneity using the state-of-art technique, i.e., Dirichlet-based label distributions. We claim that these methods fail to introduce a strong connection between data heterogeneity and the performance of the downstream task, especially computer vision tasks other then classification tasks. This undermines accurate study of the performance of current FL models for vision tasks under severe heterogeneous data scenarios. 
\end{quote}
 Our conceptual reasoning for the above claim is as follows:
\begin{quote}
As FL expands into vision tasks other than classification, there is a need to shift from simplistic, label-based data heterogeneity to approaches that recognize task-specific perspectives to the data points. In vision tasks, it is essential to model data heterogeneity in terms of how different tasks interpret and process data points. In particular, a dataset distributed across the clients in FL may appear heterogeneous from the perspective of one task but seem homogeneous from the perspective of another. 
\end{quote}
To further concertize the above reasoning, consider a vision dataset containing images of indoor scenes. In surface normal task, the goal is to predict the orientation of surfaces within the image. If clients have access only to images featuring walls or flat surfaces, the dataset may seem heterogeneous because each client’s images reflect varying surface orientations. Conversely, in depth estimation task, the same dataset can appear more homogeneous as depth estimation often relies on the spatial arrangement of objects and their relative distances rather than the orientation of surfaces. If multiple clients possess images of the same scene from different angles, the fundamental requirement -- understanding the spatial layout -- in depth estimation task remains consistent across clients, regardless of the varying surface normals. 
% Building on our claim mentioned above, in this paper, we redefines the notion of heterogeneity in FL for vision tasks. Specifically, 
To bridge this gap, in this paper, we redefine the notion of heterogeneity in FL for computer vision tasks as follows:

\begin{quote}
    Rather than inducing heterogeneity solely from a raw data perspective, we propose a migration towards a task-specific approach and assessing data heterogeneity through the unique perspective of each task to the data upon performing task-specific transformation on data.
\end{quote}

To achieve the above objective, we leverage per-trained deep neural networks (DNNs) for each tasks and feed forward data points through this network. The initial layers of the DNN of each task extract low-level features, such as edges and textures. As the data progresses through deeper layers, the network extracts higher-level representations, including shapes and patterns, that are increasingly specific to the vision task of interest. As we reach the layer just prior to the last layer (i.e, penultimate layer), embeddings that encapsulate a comprehensive view of the data from the perspective of the task are obtained, integrating both low-level and high-level features. We then leverage K-means to cluster datapoints based on their their embeddings. Subsequently, we utilize a Dirichlet distribution to assign data points of each cluster to different clients. 

% We then apply Principal Component Analysis (PCA) to these embeddings to reduce dimensionality. PCA allows us to condense the rich information contained within the embeddings into a more manageable form, preserving the most significant variance in the data while eliminating redundant features.

% after transforming data by each tasks and measuring heterogeneity from the prespective of tasks.



% To address the limitations of conventional approaches, this paper redefines heterogeneity in federated learning (FL) specifically for computer vision tasks by introducing a framework for task-specific heterogeneity. Rather than inducing heterogeneity solely from a data-level perspective before task processing, we propose a shift towards measuring heterogeneity post-transformation, examining data through the unique lens of each task’s interpretation. This approach provides a nuanced view of heterogeneity that aligns with task-specific requirements, capturing variations that emerge only when data is processed in the context of particular vision tasks.


% This new paradigm focuses on how different tasks transform the data after processing, capturing heterogeneity from a task perspective. By doing so, we move away from purely data-level heterogeneity, which only partially addresses the complexity of real-world visual tasks in FL settings, and instead adopt a comprehensive view that considers task-specific transformations.

% This approach marks the first comprehensive application of task-specific heterogeneity to FL for vision applications, addressing the unique demands of multi-task FL by accounting for the interplay of data and tasks across supervised, semi-supervised, and unsupervised learning settings. Our framework, which generalizes to classification settings as a special case, provides a flexible and robust foundation for handling non-i.i.d. data in multi-task learning environments. By addressing task-induced heterogeneity, we enable FL models to better adapt to the complexities of real-world, multi-task visual data, ultimately enhancing model performance across diverse FL scenarios.    



% These approaches do not address the intricate complexities of task-specific data heterogeneity, thereby falling short of effectively simulating realistic data conditions within FL frameworks.

% Relying solely on label-based Dirichlet distributions is insufficient to impose realistic heterogeneity for these vision tasks, as it does not adequately reflect the diverse feature dependencies that real-world vision models encounter.

% As we delve into multi-task learning, the primary objective is to identify the relationships and shared knowledge among tasks. In centralized learning settings, this is facilitated by having access to the entirety of the dataset, allowing for a holistic view that captures task interdependencies effectively. However, in the context of FL, this endeavor becomes non-trivial due to the heterogeneity of data distributed among clients. Each client may possess vastly different data distributions that influence how tasks can learn from one another, complicating the extraction of shared knowledge across tasks.

% There is a growing body of literature aiming to address these challenges; however, many of these works rely on Dirichlet distributions applied to label distributions. This approach is fundamentally flawed because it overlooks a critical aspect: the need for a paradigm shift that emphasizes examining data from the perspective of the tasks rather than just focusing on labels. In multi-task federated learning, it is essential to model data heterogeneity based on how tasks interpret and process data, as this influences learning outcomes significantly.

% Computer vision tasks, including tasks such as image classification, object detection, and segmentation, often contain complex feature interdependencies, requiring more sophisticated handling of data heterogeneity beyond label distributions.
    
% , as this influences learning outcomes significantly. 

% Here, it is essential to model data heterogeneity based on how different tasks interpret and process data, as this influences learning outcomes significantly. Specifically, in the context of computer vision, datasets can be significantly heterogeneous from the perspective of task, while they can be homogeneous from the perspective of the another task.


% It is essential to model data heterogeneity in terms of how each task interprets and processes data, as this directly impacts learning outcomes. In computer vision, for instance, a dataset may appear heterogeneous when viewed from the perspective of one task but seem homogeneous from the perspective of another. This distinction highlights the need for task-specific modeling of heterogeneity to better capture the complexities and nuances involved in multi-task federated learning.


% For example, consider a dataset of urban scenes that includes objects such as cars, pedestrians, and traffic signs. In a classification task, a client dataset containing only car images introduces heterogeneity, as the model must learn to generalize to other object types. In contrast, for an object detection task that requires identifying multiple objects within a single image, this dataset may appear more homogeneous, since all images focus on similar object types, limiting exposure to the broader data diversity necessary for generalization.



% In this work, 


% In multi-task setting, we are interested in finding the relationships among task. 

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/2_literature_review.tex <==
\section{Literature Review}

\cite{qu2022rethinking}

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/3_method.tex <==
\section{Background and Preliminaries}

\subsection{Federated System Modeling}
\subsubsection{Network Model}
We consider executing FL over a set of clients denoted by $\mathcal{N}$. Each client $n \in \mathcal{N}$ trains its local model on its local dataset  $\mathcal{D}_n$ with size $D_n = |\mathcal{D}_n|$. We also let  $\mathcal{D} = \bigcup_{n \in \mathcal{N}} \mathcal{D}_n$ with size $D = |\mathcal{D}|=\sum_{n\in\mathcal{N}}D_n$ denote the global dataset, encompassing the datasets distributed across the clients.  For an ML task of interest, we let $\ell(\bm{\omega};d)$ denote the loss of the task under arbitrary ML model parameter $\bm{\omega}$ and datapoint $d$. Subsequently, the local loss function of each client $n$ is given by $\mathcal{L}_n(\omega)=\frac{1}{D_n}\sum_{d\in\mathcal{D}_n} \ell(\bm{\omega};d)$. The goal of FL is to find the optimal model parameter to minimize the global function $\mathcal{L}(\omega)=\frac{1}{D}\sum_{d\in\mathcal{D}} \ell(\bm{\omega};d)$ for each ML task of interest, which can be mathematically represented as
\begin{equation}
    \bm{\omega}^\star = \argmin_{\bm{\omega}} \mathcal{L}(\omega) \equiv \argmin_{\bm{\omega}} \sum_{n \in \mathcal{N}}\frac{D_n \mathcal{L}_n(\omega_g)}{D}.
\end{equation}

To achieve $\bm{\omega}^\star$, FL follows an iterative approach consisting of a series of local model training at the clients and global model aggregations at the server. In particular, during each FL global aggregation round $t \in \{0,\cdots,T-1\}$, the global model, $\bm{\omega}^{(t)}$, preserved at the central server, is first broadcasted to all clients ($\bm{\omega}^{(0)}$ is often randomly initialized). Each client $n$ will then initialized its local model with the global model  as
$\bm{\omega}_n^{(t),0}~=~\bm{\omega}^{(t)}$ and
perform $K$ rounds of local ML model training via mini-batch stochastic gradient decent (SGD), each indexed by $k$, where $1\leq k\leq K$. In particular, the local model of client $n$ at the $k$-th SGD iterations during the global aggregation round $t$ is given by:
\begin{equation}
    \bm{\omega}_n^{(t), k} = \bm{\omega}_n^{(t),k-1} - \eta^{(t), k}_n\widetilde{\nabla}\mathcal{L}_n(\bm{\omega}_n^{(t),k-1}),
\end{equation}
where $\eta^{(t), k}_n$ is the instantaneous learning-rate. Also, $\widetilde{\nabla}$ denotes the stochastic gradient approximation defined as  $\widetilde{\nabla}\mathcal{L}_n(\bm{\omega}_n^{(t),k-1}) =  \frac{1}{|\mathcal{B}_n^{(t), k-1}|} \sum_{d \in \mathcal{B}_n^{(t), k-1}} \nabla \ell(\bm{\omega}_n^{(t),k-1};d)$, where $\mathcal{B}_n^{(t), k-1}\subseteq \mathcal{D}_n$ represents the set of sampled datapoints contained in the mini-batch.





After the conclusion of local model training, clients send their latest trained local ML models (i.e.,  $\bm{\omega}_n^{(t), K}$ for each client $n$) to the server, where the received models are aggregated to create a new global model as follows:
\begin{equation}
    \bm{\omega}^{(t+1)} = \sum_{n\in\mathcal{N}} \frac{D_n \bm{\omega}_n^{(t),K}}{D}.
\end{equation}
This new global model is then broadcasted back to the clients to start the next local model training round and this iterative procedure is repeated until desired convergence is achieved.  
Note that the procedure formulated above describes the vanilla FedAvg method {\color{red}[CITE]}. Other variation of FL, which are studied later in Sec.~4, often involve modifications to the above-described local training and global aggregation processes.

% \subsubsection{Local ML Model Training}
% After the model is broadcasted to the clients ($\omega_n^{(t),0}~=~\omega_g^{(t)}, \forall n \in \mathcal{N}$), each client trains their local ML model for $K$ rounds using the update formula below
% \begin{equation}
%     \omega_n^{(t), k} = \omega_n^{(t),k-1} - \eta^{(t), k}_n\widetilde{\nabla}\mathcal{L}_n(\omega_n^{(t),k-1}), \forall k \in [0, K],
% \end{equation}
% where in federated round $t$ and local training round $k$, $\omega_n^{(t),k}$ represents the client's ML model parameters, $\eta^{(t), k}_n$ is the client's learning rate, and $\widetilde{\nabla}\mathcal{L}_n(\omega_n^{(t),k-1})$ is the stochastic gradient of the loss function $\mathcal{L}$ used to train client $n$ on its corresponding task with the model parameters $\omega_n^{(t),k-1}$ on a random minibatch of data. The stochastic gradient can be acquired via  
% \begin{equation}
% \begin{aligned}
%     \widetilde{\nabla}\mathcal{L}_n(\omega^{(t), k}_n) & = \widetilde{\nabla}\mathcal{L}_n(\omega^{(t), k}_n; \mathcal{B}_n^{(t), k}) \\
%     & \triangleq \frac{1}{|\mathcal{B}_n^{(t), k}|} \sum_{d \in \mathcal{B}_n^{(t), k}} \nabla \ell(\omega^{(t), k}_n; d),
% \end{aligned}
% \end{equation}
% where $\mathcal{B}_n^{(t), k}$ represents a minibatch of data randomly sampled at global round $t$ and local round $k$ from client $n$'s local dataset $\mathcal{D}_n$. After the K-th local ML model training round is finished for all clients, the model parameters $\omega_n^{(t), K}, \forall n \in \mathcal{N}$ are sent in the uplink transmission to the server.

% The objective function we define in this problem setting is the average loss of the global model on the clients' respective datasets which can be mathematically shown through

% \begin{equation}
%     \omega_g^\star = \argmin_{\omega_g} \sum_{n \in \mathcal{N}}\frac{D_n \mathcal{L}_n(\omega_g)}{D}.
% \end{equation}

% \subsubsection{Global Model Aggregation}
% After the server receives the uplink transmissions from the clients, the local ML models are aggregated to create the new global model which is acquired as

% \begin{equation}
%     \omega_g^{(t+1)} = \sum_{n\in\mathcal{N}} \frac{D_n \omega_n^{(t),K}}{D}
% \end{equation}

% The new global model will be then broadcasted to all clients in the network to perform another round of local ML model training.

% \begin{equation}
%     {\omega_g}^{(t+1)} = \frac{\sum_{n\in\mathcal{N}} D_n \omega_{n}^{(t),K} {\sum_{n\in\mathcal{N}} |\mathcal{D}_n|}
% \end{equation}

\subsection{Current Approaches on Modeling Heterogeneity} \label{sec:dirichlet-approach}

In the state-of-the-art in FL for visual tasks {\color{red}[CITE]}, simulations that model data heterogeneity across the clients, have heavily relied on classification where the creation of data heterogeneity is possible through label distribution. From trivial approaches such as partially distributing the labels across clients (i.e., each client has only a share of the available labels in the dataset) {\color{red} [CITE]} to more theoretically-oriented approaches such as utilizing Dirichlet distribution {\color{red} [CITE]}, most of the previously developed methods concern the ratio of the class labels and therefore will be concerning heterogeneity in vision classification tasks.
The first question that we want to answer when tackling the notion of heterogeneity in non-classification vision tasks would be \textit{``Does the difference in label ratio affect the non-classification tasks to the same extent as classification tasks?"}
To answer this question, we propose an experiment for a set of non-classification tasks, where we employ the Dirichlet distribution to create various ratios for each client's local dataset from each class label. We then compare the performance of FL under the induced heterogeneity to measure the extent of data heterogeneity's effect when only concerning extracted image classes.

\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.24\textwidth]{author-kit-CVPR2025-v3.1-latex-/figs/alpha_values/dirichlet_distribution_1000000.pdf}
    \includegraphics[width=0.24\textwidth]{author-kit-CVPR2025-v3.1-latex-/figs/alpha_values/dirichlet_distribution_1000.pdf}
    \includegraphics[width=0.24\textwidth]{author-kit-CVPR2025-v3.1-latex-/figs/alpha_values/dirichlet_distribution_10.pdf}
    \includegraphics[width=0.24\textwidth]{author-kit-CVPR2025-v3.1-latex-/figs/alpha_values/dirichlet_distribution_0.1.pdf}
    \caption{Dirichlet-generated distribution probabilities for $N = 20$ clients and 16 classes with homogeneous prior probabilities (i.e., $p_c = 1/|\mathcal{C}|$). In the case of $\alpha=10^6$, the data is homogeneously distributed across clients, whereas in the case of $\alpha=0.1$, the majority of each client's data is consisted of two labels at most. The decrease in the homogeneity of the clients' data is also observed by comparing the distribution probabilities generated given $\alpha=10^3$ and $\alpha=10$.}
    \label{fig:alpha-values}
\end{figure*}

\subsubsection{Dirichlet Distribution}
Given a set of classification labels $\mathcal{C} = \{c_i\}_{1\leq i \leq |\mathcal{C}|}$, where $c_i$ denotes the $i$-th label in the dataset\footnote{e.g., the digits in MNIST \cite{mnist}}, we can distribute the labels across multiple devices by creating a distribution vector $\mathbf{q}$ based on the Dirichlet distribution $\mathsf{Dir}(\alpha\mathbf{p})$. Here, $\mathbf{p} = \{p_c\}_{c\in\mathcal{C}}$ stands for the prior distribution of the data for each class $c$ which in our case is the original distribution of the classes, and $\alpha > 0$ is the concentration parameter which determines how closely the distribution vector resembles the prior distribution. Creating a distribution vector $\mathbf{q}_n$ for each client $n$ will result in $N = |\mathcal{N}|$ independent distribution probability vectors to form each client's dataset from the $\mathcal{C}$ classification labels. Increasing in the concentration parameter $\alpha$ will lead to a more \textit{homogeneously distributed} set of vectors, as they will resemble the prior distribution to a higher extent. The visualization of this phenomenon is included in Fig. \ref{fig:alpha-values}. 

\subsubsection{Testing non-Classification Tasks Under a classification-based Heterogeneity}
Utilizing the Dirichlet distribution to create a heterogeneous setting for the clients' local datasets, we will experiment with non-classification tasks while inducing heterogeneity based on a categorical attribute of the images, i.e., class. We use the well-recognized Taskonomy~\cite{taskonomy} dataset for our simulations due to the variety in classification and non-classification tasks and the existing labels for each task on each image.
We distribute the data across clients based on the original distribution of the ``class\_scene" class provided in the dataset which are in the form of probabilities for each class from which we take the highest probability as the assigned class to each specific image. We then experiment with the non-classification tasks to observe the change in performance in a federated scenario. As the data heterogeneity increases, the performance of the federated system (i.e., the loss of the global model) should worsen (converge to a higher value). We conduct these experiments in each network with one task only, and consider the tasks ``edge\_texture," ``reshading," ``normal," ``segment\_semantic," and ``keypoints3d." We then plot the results of each task across various concentration parameters to account for different levels of heterogeneity. The results of this experiment are shown in Fig. \ref{fig:embedding-vs-class}. The results of the scene classification task are also included for comparison across the other tasks and the original task to which the heterogeneous distribution correspond.

\begin{figure*}[!h]
    \centering
    \includegraphics[width=\textwidth]{author-kit-CVPR2025-v3.1-latex-/figs/fedavg_class_vs_embedding.jpeg}
    \caption{Comparison of how performing Dirichlet distribution over the ``scene\_class" feature and the extracted embeddings affect the performance in FL. As it is shown, distributing the datapoints based on the class of the scene they correspond to has not resulted in a significant change in the performance across various values of $\alpha$. However, distributing the datapoints based on the clusters formed by the extracted embeddings with the Dirichlet distributions of various $\alpha$ parameters has created a performance gap across the possible scenarios with the $\alpha=0.1$ (most heterogeneous case) resulting in the worst performance and $\alpha=1000$ (least heterogeneous case) resulting in the best performance.}
    \label{fig:embedding-vs-class}
\end{figure*}

The plots show that no specific pattern is shaped in any of the non-classification tasks with increasing the value of $\alpha$ which is contrary to what was shown in \cite{fl-dirichlet} to happen in the case of visual classification tasks. However, oGiven the incoherency between the expected results in the case where heterogeneity affects the performance and our observations in the case of non-classification tasks, we can conclude that the induced heterogeneity -which is based on classes- does not affect the results of another non-classification task. Thus, a research gap in extending the notion of heterogeneity to a more general form can be assumed.

==> sec/4_task_het.tex <==
\section{Data Heterogeneity from Task Perspective}
As the need for an extensive notion of heterogeneity was presented, we attempted to first view the problem from a task's perspective which was to follow the leads one task can provide into how data can be "heterogeneous" \textit{from the task's viewpoint}. Since a ``class label" represents a feature that can group various datapoints, we aimed to find the same utility in tasks that do not possess it beforehand: non-classifying tasks do not possess a class, and grouping the data into clusters based on their original high-level features such as RGB values would not gain a \textit{task-specific} information regarding heterogeneity. Therefore, we need to first find a source of information that specifically belongs to the task being trained.

\subsection{Finding a task-specific source of information}
Going back to the architecture of a neural network, we aimed to extract the task-specific information from the penultimate layer of the neural network being trained on a task. As shown in Fig. \ref{---} {\color{red} ADD FIGURE}, we consider two major sections in a neural network's architecture: The \textit{encoder} which extracts the features from the input image, and the \textit{decoder} which performs manipulations on the extracted features to create the desired output for a specific task. We assume that the last layer of the decoder performs translation from the mid-level feature space into the output domain, and therefore separate it from other parts of the decoder into an ``output layer." The input to the output layer can then be regarded as the richest information available that describes a datapoint being passed through a network from the task's perspective. We will recall these features as \textit{embeddings} for the remainder of this discussion.

\subsection{Clustering the data for a specific task}
After finding the information that best describes datapoints from the task's perspective, we aim to cluster our datapoints based on their embeddings to create multiple clusters that can act analogous to the clusters of labels in classification tasks. To this end, we utilize \textit{k-means clustering} to cluster the extracted embeddings. We performed the clustering for the embeddings of datapoints trained on the scene classification task in the taskonomy dataset which are presented in Fig. \ref{fig:scene-class-embedding-clusters}.
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.49\textwidth]{author-kit-CVPR2025-v3.1-latex-/figs/tsne_scene_class.pdf}
    \caption{Embedding clusters extracted from the scene classification task model. Each color represents a specific class.}
    \label{fig:scene-class-embedding-clusters}
\end{figure}
It is shown that the embeddings from each specific scene class are sorted into separable clusters which also correspond to their respective classes. This raises confidence in the statement ``The embeddings describe the datapoints from a task's perspective."

\subsection{Creating heterogeneous local datasets for clients}
Having the clusters, we can now create the local datasets $\mathcal{D}_n$ for each client $n$. We can then repeat Sec. \ref{sec:dirichlet-approach} experiments to measure the effect of the induced heterogeneity by replacing the class clusters with the embedding clusters. The prior distribution of classes $\mathbf{p}$ is now replaced by the distribution of the embeddings in each cluster $\mathbf{p}_{e}$. Therefore, the probability distribution of classes for each client $\mathbf{q}_n$ will also be replaced with the probability distribution of embedding clusters $\mathbf{q}_{n,e}$. The clients will then be assigned data from each cluster based on their own $\mathbf{q}_{n,e}$ and train the global model in a federated fashion. We have experimented with the same tasks in Sec. \ref{sec:dirichlet-approach} and included the results in Fig. \ref{fig:embedding-vs-class}.
Our results show that the global model loss on each client's dataset converges to a higher value as we increase the heterogeneity (decrease the parameter $\alpha$) across experiments of the same task. This observation falls in line with our initial hypothesis regarding the effect of heterogeneity on the performance of the federated system. We can thus deduce that a task-specific heterogeneity can be more effective in modeling a heterogeneous federated system instead of a class-based heterogeneity which has been used in the prior literature in FL \cite{qu2022rethinking, mendieta2022local, NEURIPS2021_2f2b2656, fl-dirichlet}.

==> sec/5_benchmarks.tex <==
\begin{table*}[!h]
    \centering
    \begin{tabularx}{\textwidth}{ 
      | >{\centering\arraybackslash}m{26.5mm} 
      | >{\centering\arraybackslash}m{13mm}
      | >{\centering\arraybackslash}X 
      | >{\centering\arraybackslash}X 
      | >{\centering\arraybackslash}m{19mm} 
      | >{\centering\arraybackslash}X 
      | >{\centering\arraybackslash}m{20mm} 
      | >{\centering\arraybackslash}X 
      | >{\centering\arraybackslash}X|} 
        \hline
         Task & \diagbox[width=17.5mm]{$\alpha$}{Method\hspace{-1.5mm}} & FedAvg & FedProx & {SCAFFOLD} & FedPer & FedGradNorm & Ditto & FedSTA\\
        \hline
        \multirow{3}{*}{edge\_texture}
         & 0.1 & & & & & & &\\
         & 10 & & & & & & &\\
         & 1000 & & & & & & &\\
        \hline
        \multirow{3}{*}{normal}
         & 0.1 & & & & & & &\\
         & 10 & & & & & & &\\
         & 1000 & & & & & & &\\
        \hline
        \multirow{3}{*}{reshading}
         & 0.1 & & & & & & &\\
         & 10 & & & & & & &\\
         & 1000 & & & & & & &\\
        \hline
        \multirow{3}{*}{segment\_semantic}
         & 0.1 & & & & & & &\\
         & 10 & & & & & & &\\
         & 1000 & & & & & & &\\
        \hline
        \multirow{3}{*}{inpainting}
         & 0.1 & & & & & & &\\
         & 10 & & & & & & &\\
         & 1000 & & & & & & &\\
        \hline
        \multirow{3}{*}{keypoints3d}
         & 0.1 & & & & & & &\\
         & 10 & & & & & & &\\
         & 1000 & & & & & & &\\
        \hline
        \multirow{3}{*}{depth\_euclidean}
         & 0.1 & & & & & & &\\
         & 10 & & & & & & &\\
         & 1000 & & & & & & &\\
        \hline
        \multirow{3}{*}{principal\_curvature}
         & 0.1 & & & & & & &\\
         & 10 & & & & & & &\\
         & 1000 & & & & & & &\\
        \hline
        \multirow{3}{*}{class\_scene}
         & 0.1 & & & & & & &\\
         & 10 & & & & & & &\\
         & 1000 & & & & & & &\\
        \hline
    \end{tabularx}
    \caption{Caption}
    \label{tab:benchmark}
\end{table*}

\section{Benchmarks}
In this section, we experiment with the common methods in FL to provide a benchmark for the performance of FL under task-specific heterogeneity. 



%%% To ensure keeping various image types (1-channel/BW vs. 3-channel/RGB) and various classification objectives (digit/object/scene) into consideration, we experiment with three datasets of MNIST\cite{mnist} (BW-handwritten igits), CIFAR10\cite{cifar10} (RGB-object), and Taskonomy\cite{taskonomy} (RGB-scene class).

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.5\linewidth]{author-kit-CVPR2025-v3.1-latex-/figs/embedding_to_class_mnist.jpeg} \\
    \includegraphics[width=0.5\linewidth]{author-kit-CVPR2025-v3.1-latex-/figs/embedding_to_class_mnist.jpeg} \\
    \caption{Top: Clustering the extracted embeddings with k-means has shown that the datapoints belonging to each class will subsequently be clustered together. This is our starting point to explore the capabilities that the information from the embeddings can provide when gazing at data heterogeneity from each task's perspective. Bottom: The same plot is acquired for the ``scene\_class" classification task in the Taskonomy dataset. The datapoints belonging to the same scene class are clustered together. This shows that the embedding feature space is not only useful when dealing with 1-channel (grayscale) images, but in more complex input feature spaces such as RGB as well.}
    \label{fig:embedding_to_class_mnist}
\end{figure}



